A Primer on the Inner Workings of Transformer-based Language Models

The rapid progress of research aimed at interpreting the inner workings of advanced language models has highlighted a need for contextualizing the insights gained from years of work in this area. This primer provides a concise technical introduction to the current techniques used to interpret the inner workings of Transformer-based language models, focusing on the generative decoder-only architecture. We conclude by presenting a comprehensive overview of the known internal mechanisms implemented by these models, uncovering connections across popular approaches and active research directions in this area.

==> figures/overview-table.tex <==
\begin{tikzpicture}[
    every text node part/.style={align=center},
    category/.style={rectangle, fill=white, anchor=center, xshift=-0.5mm},
    title/.style={rectangle, fill=black!2, anchor=center},
    content/.style={rectangle, fill=black, opacity=1, fill opacity=0.06, text opacity=1, anchor=center},
    >={Latex[width=1.5mm,length=1.5mm]},
]
\large
\pgfmathsetmacro{\tmargin}{0.1}
\pgfmathsetmacro{\tboxwidth}{2.5}
\pgfmathsetmacro{\tboxheight}{0.985}
\pgfmathsetmacro{\tcategoryheight}{0.3}
\pgfmathsetmacro{\tcategoryrelfontsize}{-1}

\newcommand{\pref}[2]{#1 \hyperref[#2]{§\,\ref*{#2}}}

\newcommand{\rAs}{\rBe + \tmargin} \newcommand{\rAe}{\rAs + \tboxheight}
\newcommand{\rBs}{\rCe + \tmargin} \newcommand{\rBe}{\rBs + \tboxheight}
\newcommand{\rCs}{\rDe + \tmargin} \newcommand{\rCe}{\rCs + \tboxheight}
\newcommand{\rDs}{\rEe + \tmargin} \newcommand{\rDe}{\rDs + \tboxheight}
\newcommand{\rEs}{\rFe + \tmargin + \tcategoryheight + \tmargin} \newcommand{\rEe}{\rEs + \tboxheight}
\newcommand{\rFs}{\rGe + \tmargin + \tcategoryheight + \tmargin} \newcommand{\rFe}{\rFs + \tboxheight}
\newcommand{\rGs}{\rHe + \tmargin} \newcommand{\rGe}{\rGs + \tboxheight}
\newcommand{\rHs}{\rIe + \tmargin} \newcommand{\rHe}{\rHs + \tboxheight}
\newcommand{\rIs}{\rJe + \tmargin} \newcommand{\rIe}{\rIs + \tboxheight}
\newcommand{\rJs}{\tmargin} \newcommand{\rJe}{\rJs + \tboxheight}

\newcommand{\cAs}{\tmargin} \newcommand{\cAe}{\cAs + \tboxwidth}
\newcommand{\cBs}{\cAe + \tmargin} \newcommand{\cBe}{\cBs + \tboxwidth}
\newcommand{\cCs}{\cBe + \tmargin} \newcommand{\cCe}{\cCs + \tboxwidth}
\newcommand{\cDs}{\cCe + \tmargin} \newcommand{\cDe}{\cDs + \tboxwidth}
\newcommand{\cEs}{\cDe + \tmargin} \newcommand{\cEe}{\cEs + \tboxwidth}
\newcommand{\cFs}{\cEe + \tmargin + \tmargin} \newcommand{\cFe}{\cFs + \tboxwidth}

\newcommand{\rtitle}[2]{
    \fill[title] (-\tmargin-\tboxwidth, \csname r#1s\endcsname) rectangle node{\vphantom{$^i_ a$}#2\vphantom{$^i_a$}} (-\tmargin, \csname r#1e\endcsname);
}
\newcommand{\rcategory}[2]{
    \fill[category] (-\tmargin-\tboxwidth, \csname r#1e\endcsname + \tmargin + \tcategoryheight) rectangle node{\relsize{\tcategoryrelfontsize} #2} (-\tmargin, \csname r#1e\endcsname + \tmargin);
    \draw (\cAs, \csname r#1e\endcsname + \tmargin) -- (\cEe, \csname r#1e\endcsname + \tmargin);
    \draw (\cFs, \csname r#1e\endcsname + \tmargin) -- (\cFe, \csname r#1e\endcsname + \tmargin);
}

\newcommand{\ctitle}[2]{
    \fill[title] (\csname c#1s\endcsname, \rAe + \tmargin + \tmargin) rectangle node{\vphantom{$^i_ a$}#2\vphantom{$^i_a$}} (\csname c#1e\endcsname, \rAe + \tmargin + \tmargin + \tboxheight);
}
\newcommand{\ccategory}[2]{
    \fill[category] (\csname c#1s\endcsname, \rAe + \tmargin + \tmargin + \tboxheight + \tmargin + \tcategoryheight) rectangle node{\relsize{\tcategoryrelfontsize} #2} (\csname c#1e\endcsname, \rAe + \tmargin + \tmargin + \tboxheight + \tmargin);
    \draw (\csname c#1s\endcsname - \tmargin, \rJs) -- (\csname c#1s\endcsname - \tmargin, \rAe);
}

\newcommand{\tcontent}[4]{
    \fill[content] (\csname c#2s\endcsname, \csname r#1s\endcsname) rectangle node{\vphantom{$^i_ a$}#4\vphantom{$^i_a$}} (\csname c#3e\endcsname, \csname r#1e\endcsname);
}

%\draw[->] (\cAs, \rAe + \tmargin + \tmargin + \tboxheight + \tcategoryheight + \tmargin + \tmargin) -- (\cFe, \rAe + \tmargin + \tmargin + \tboxheight + \tcategoryheight + \tmargin + \tmargin) node[above left, xshift=-0.2cm]{less information \hspace{9.3cm} more information};

%\draw[->] (\cAs - \tmargin - \tmargin - \tboxwidth - \tmargin, \rAe) -- (\cAs - \tmargin - \tmargin - \tboxwidth - \tmargin, \rJs) node[anchor=mid, below, rotate=-90, xshift=-6cm]{lower abstraction \hspace{5cm} higher abstraction};

\rcategory{A}{local explanation}
\rtitle{A}{input \\ features}
\rtitle{B}{adversarial \\ examples}
\rtitle{C}{influential \\ examples}
\rtitle{D}{counter-\\factuals}
\rtitle{E}{natural \\ language}
\rcategory{F}{class explanation}
\rtitle{F}{concepts}
\rcategory{G}{global explanation}
\rtitle{G}{vocabulary}
\rtitle{H}{ensemble}
\rtitle{I}{linguistic \\ information}
\rtitle{J}{rules}

\%ccategory{A}{post-hoc \hspace{0.9cm}}
\ctitle{A}{black-box}
\ctitle{B}{dataset}
\ctitle{C}{gradient}
\ctitle{D}{embeddings}
\ctitle{E}{white-box}
%\ccategory{F}{intrinsic \hspace{1.1cm}}
\ctitle{F}{model specific}

\tcontent{A}{A}{A}{\pref{SHAP}{sec:input-features:shap}}
\tcontent{A}{A}{B}{\hspace{2.1cm}\pref{LIME}{sec:input-features:lime},\\\hspace{2.1cm}\pref{Anchors}{sec:input-features:anchors}}
\tcontent{A}{C}{C}{\pref{Gradient}{sec:input-features:gradient},\\ \pref{IG}{sec:input-features:integrated-gradient}}
\tcontent{A}{F}{F}{Attention}
\tcontent{B}{A}{A}{\pref{SEA$^\mathcal{M}$}{sec:adversarial-examples:sea}}
\tcontent{B}{C}{D}{\pref{HotFlip}{sec:adversarial-examples:hotflip}}
\tcontent{C}{B}{C}{\pref{Influence Functions$^\mathcal{H}$}{sec:influential-examples:influence-functions}\\\pref{TracIn$^\mathcal{C}$}{sec:influencial-examples:tracin}}
\tcontent{C}{B}{E}{\hspace{4.3cm} \pref{Representer Pointers$^{\dagger}$}{sec:influential-examples:representer-point-selection}}
\tcontent{C}{F}{F}{Prototype \\ Networks}
\tcontent{D}{A}{A}{\pref{Polyjuice$^{\mathcal{M},\mathcal{D}}$\\}{sec:counterfactuals:polyjuice}}
\tcontent{D}{A}{C}{\pref{MiCE$^\mathcal{M}$}{sec:counterfactuals:mice}}
\tcontent{E}{A}{A}{\pref{CAGE$^{\mathcal{M},\mathcal{D}}$\\}{sec:natural-language:cage}}
\tcontent{E}{F}{F}{GEF$^{\mathcal{D}}$, NILE$^\mathcal{D}$}

%\tcontent{F}{A}{A}{\pref{Total Effect$^\mathcal{D}$\\}{sec:concepts:total-effect}}
%\tcontent{F}{E}{E}{\pref{Natural\\ Effect$^\mathcal{D}$}{sec:concepts:natural-effect}}
\tcontent{F}{E}{E}{\pref{NIE$^\mathcal{D}$}{sec:concepts:natural-indirect-effect}}

\tcontent{G}{D}{D}{\pref{Project}{sec:vocabulary:projection},\\ \pref{Rotate}{sec:vocabulary:rotation}}
\tcontent{H}{A}{B}{\pref{SP-LIME}{sec:ensemble:sp-lime}}
\tcontent{I}{A}{A}{\pref{Behavioral\\ Probes$^\mathcal{D}$}{sec:linguistic-information:behavioral-probes}}
\tcontent{I}{D}{D}{\pref{Structural \\ Probes$^\mathcal{D}$}{sec:linguistic-information:structural-probes}}
\tcontent{I}{E}{E}{\pref{Structural \\ Probes$^\mathcal{D}$}{sec:linguistic-information:structural-probes}}
\tcontent{I}{F}{F}{Auxiliary \\ Task$^\mathcal{D}$}
\tcontent{J}{A}{B}{\pref{SEAR$^\mathcal{M}$}{sec:rules:sear}}
\tcontent{J}{B}{E}{\pref{Compositional Explanations of Neurons$^{\dagger}$}{sec:rules:comp-explain-neuron}}

\end{tikzpicture}

==> figures/toc-diagram.tex <==
\definecolor{grey_4}{HTML}{808080}
\definecolor{grey_3}{HTML}{B3B3B3}
\definecolor{grey_2}{HTML}{CCCCCC}
\definecolor{grey_1}{HTML}{E6E6E6}

\definecolor{red_4}{HTML}{993939}
\definecolor{red_3}{HTML}{ED9595}
\definecolor{red_2}{HTML}{FF9999}
\definecolor{red_1}{HTML}{F8CECC}

\definecolor{blue_4}{HTML}{6C8EBF}
\definecolor{blue_3}{HTML}{92BAE8}
\definecolor{blue_2}{HTML}{DAE8FC}
\definecolor{white_grey}{HTML}{DEDEDE}
%\tikzstyle{edge from parent}=[draw]
%\large
\begin{tikzpicture}[grow cyclic, shape=circle, text width=2.5cm, align=flush center, every node/.style=concept, concept color=white_grey,
level 1/.style={level distance=5cm,sibling angle=90},
level 2/.style={level distance=4cm,sibling angle=60},
edge from parent/.style={draw,-}]

\newcommand{\pref}[2]{#1 \hyperref[#2]{§\,\ref*{#2}}}

\node{\textbf{\large{Inner Workings of Transformer LMs}}} [clockwise from=90]  % root node
   child [concept color=teal!30] { node {\pref{\textbf{Components of a Transformer LM}}{sec:components_transformer_lm}}[clockwise from=110]
        child [concept color=teal!30] { node {\pref{The Transformer Layer}{sec:transformer_layer}} 
            }
        child [concept color=teal!30] { node {\pref{Prediction Head and Linearity of Transformers}{sec:prediction_head}}}
    }
    child [concept color=blue_3] { node {\pref{\textbf{Behavior Localization}}{sec:behavior_localization}}  [clockwise from=60]
        child [concept color=blue_3] { node {\pref{Input Attribution}{sec:input_attribution}}}
        child [concept color=blue_3] { node {\pref{Model Component Importance}{sec:components_importance}}}
    }
    child [concept color=red_3] { node {\pref{\textbf{Known Inner Behaviors}}{sec:what_we_know_transformer}}  [counterclockwise from=180]
        child [concept color=red_3] { node {\pref{Attention Block}{sec:insights_attention}}}
        child [concept color=red_3] { node {\pref{Feedforward Network}{sec:insights_ffn}}}
        child [concept color=red_3] { node {\pref{Residual Stream}{sec:insights_res_stream}}}
        child [concept color=red_3] { node {\pref{Emergent Multi-component Behavior}{sec:emergent_behaviors}}}
    }
    child [concept color=green_drawio] { node {\pref{\textbf{Information Decoding}}{sec:information_decoding}}  [counterclockwise from=60]
        child [concept color=green_drawio] { node {\pref{Probing}{sec:probing}}}
        child [concept color=green_drawio] { node {\pref{Linear Representation Hypothesis}{sec:linear_rep_hypothesis}}}
        child [concept color=green_drawio] { node {\pref{Sparse Autoencoders}{sec:saes}}}
        child [concept color=green_drawio] { node {\pref{Decoding in Vocabulary Space}{sec:token_space}}}  
    };

\end{tikzpicture}
